Techniques for Continuous Touch-Based Authentication Modeling

The field of touch-based authentication has been rapidly developing over the last decade, creating a fragmented and difficult-to-navigate area for researchers and application developers alike due to the variety of methods investigated. In this study, we perform a systematic literature analysis of 30 studies on the techniques used for feature extraction, classification, and aggregation in touch-based authentication systems as well as the performance metrics reported by each study. Based on our findings, we design a set of experiments to compare the performance of the most frequently used techniques in the field under clearly defined conditions. In addition, we introduce three new techniques for touch-based authentication: an expanded feature set (consisting of 149 unique features), a multi-algorithm ensemble-based classifier, and a Recurrent Neural Network based stacking aggregation method. The comparison includes 14 feature sets, 11 classifiers, and 5 aggregation methods. In total, 219 model configurations are examined and we show that our novel techniques outperform the current state-of-the-art in each category. The results are also validated across three different publicly available datasets. Finally, we discuss the findings of our investigation with the aim of making the field more understandable and accessible for researchers and practitioners.

==> figures/aggregations.tex <==
\begin{figure*}[!t]
\includegraphics[width=1.00\linewidth]{images/aggregations.pdf}
\caption{Aggregations}
\label{fig:aggregations}
\end{figure*}

==> figures/classifiers.tex <==
\begin{figure*}[!t]
\includegraphics[width=1.00\linewidth]{images/classifiers.pdf}
\caption{classifiers}
\label{fig:classifiers}
\end{figure*}

==> figures/features.tex <==
\begin{figure}[!th]
\includegraphics[width=1.00\linewidth]{images/features.pdf}
\caption{Performance of featuresets under the same conditions. Our proposed feature collection (All or ANOVA feature selection) outperforms all individual featuresets proposed in related work.}
\label{fig:features}
\end{figure}

==> figures/statistics.tex <==
\begin{figure*}[!t]
	\begin{minipage}[t]{.31\textwidth}
    \includegraphics[width=1.00\linewidth]{images/classifier_statistics.pdf}
    \caption{Prevalence of classifiers}
    \label{fig:classification_statistics}
    \end{minipage}%
    \begin{subfigure}{.02\textwidth}
    \hfill
    \end{subfigure}
    \begin{minipage}[t]{.29\textwidth}
    \includegraphics[width=1\linewidth]{images/aggreagation_statistics.pdf}
    \caption{Prevalence of aggregation methods}
    \label{fig:aggregation_statistics}
    \label{fig:include_exclude_difference}
    \end{minipage}
    \begin{subfigure}{.02\textwidth}
    \hfill
    \end{subfigure}
    \begin{minipage}[t]{.32\textwidth}
    \includegraphics[width=1.00\linewidth]{images/metrics_statistics.pdf}
    \caption{Prevalence of metrics}
    \label{fig:metrics_statistics}
    \end{minipage}
\end{figure*}

==> figures/statistics_new.tex <==
\begin{figure}[!t]
\includegraphics[width=1.00\linewidth]{images/statistics.pdf}
\caption{The prevalence of use of classification models, aggregation methods and performance metrics in touch-based authentication studies.}
\label{fig:statistics}
\end{figure}

==> tables/features.tex <==
\vspace{10px}
\begin{table*}[!t]
% increase table row spacing, adjust to taste
\small
\renewcommand{\arraystretch}{1.3}
\caption{Geometric features found in related work \red{(in progress)}. perc. - pecentile, dev. - deviation, accel. - acceleration. Full details about each of the features can be found in the corresponding papers and in our publicly available source code. Note \cite{hmm-model, dictionaries, cont-auth-deep-learning} use the same as \cite{touchalytics} and \cite{swipe-gesture} uses the same as \cite{information-revealed} except the mid-stroke pressure.} 
\vspace{6px}
\label{tab:features}
\centering
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{ll|ll|ll}
\toprule
Feature & Studies & Feature & Studies & Feature & Studies
\\
\midrule
1-2. Start X,Y & \makecell[l]{\cite{touchalytics, unobservable-re-authentication, towards-continuous-passive, performance-analysis,information-revealed}\\ \cite{active-user-authentication, posture-size-config, dakota, touch-pattern-isolation}} & 39. Average acceleration & \cite{which-verifiers-work, performance-analysis} & & \\
3-4. Stop X,Y & \makecell[l]{\cite{touchalytics, towards-continuous-passive, performance-analysis, information-revealed, active-user-authentication}\\ \cite{posture-size-config, dakota, touch-pattern-isolation}} & 40. Standard Deviation pressure & \cite{which-verifiers-work, towards-continuous-passive, performance-analysis} & & \\
5. Stroke duration & \makecell[l]{\cite{touchalytics, unobservable-re-authentication, which-verifiers-work, towards-continuous-passive, performance-analysis, information-revealed}\\ \cite{power-consumption, active-user-authentication, posture-size-config, dakota, touch-pattern-isolation}} & 41. Standard Deviation area  & \cite{which-verifiers-work, towards-continuous-passive} & 73. LDP to Stop Length & \cite{towards-continuous-passive}  \\
6. End-to-end distance &  \makecell[l]{\cite{touchalytics, which-verifiers-work,  towards-continuous-passive, information-revealed, power-consumption}\\ \cite{active-user-authentication, posture-size-config, dakota, touch-pattern-isolation}} & 42. Standard Deviation velocity & \cite{which-verifiers-work, performance-analysis, active-user-authentication} & 74. LDP to Stop Direction & \cite{towards-continuous-passive} \\
7. Mid-stroke pressure & \cite{touchalytics, which-verifiers-work,  performance-analysis, information-revealed, posture-size-config, dakota} & 43. Standard Deviation acceleration & \cite{which-verifiers-work, performance-analysis} & 75. \makecell[l]{Ratio of "end to end distance"\\ and LDP length} & \cite{towards-continuous-passive}  \\
8. Mid-stroke area & \cite{touchalytics, which-verifiers-work, information-revealed, dakota} & \makecell[l]{44-47. First Quartile pressure,\\ area, velocity, acceleration} & \cite{which-verifiers-work} & 76. Total displacement length & \cite{performance-analysis}  \\
9. Length of Trajectory & \makecell[l]{\cite{touchalytics, unobservable-re-authentication, which-verifiers-work, towards-continuous-passive, performance-analysis}\\\cite{information-revealed, posture-size-config, dakota, touch-pattern-isolation}} & \makecell[l]{48-51. Third Quartile pressure,\\ area, velocity, acceleration} & \cite{which-verifiers-work} & 77. \makecell[l]{Ratio of displacement\\ and trajectory length} & \cite{performance-analysis}  \\
10. Inter-stroke time & \cite{touchalytics, active-user-authentication, posture-size-config} & 52-55. Extreme point 1,2 - X,Y & \cite{which-verifiers-work} & 78. Median distance between points & \cite{performance-analysis}   \\
11. Mean Resultant Length & \cite{touchalytics, information-revealed, active-user-authentication, dakota} & 56. Tangent between last 2 points & \cite{which-verifiers-work} & 79. IQR distance between points & \cite{performance-analysis} \\
12. Median accel. at first 5 points & \cite{touchalytics, active-user-authentication, dakota}
& 57. Velocity at first point & \cite{towards-continuous-passive} & 80. Skewness of distance between points &  \cite{performance-analysis} \\
13. Median velocity at last 3 points & \cite{touchalytics, active-user-authentication, dakota} &  \makecell[l]{58-60. Area, Pressure,\\ Velocity at last point} & \cite{towards-continuous-passive} & 81. Kurtosis of distance between points & \cite{performance-analysis}  \\
14. Average velocity & \makecell[l]{\cite{touchalytics, which-verifiers-work,  towards-continuous-passive, performance-analysis}\\\cite{information-revealed, posture-size-config, dakota, touch-pattern-isolation}} & 61. Last moving direction & \cite{towards-continuous-passive} & 82. Average end-to-end dev.  & \cite{performance-analysis} \\
15. Up/Down/Left/Right flag & \cite{touchalytics, information-revealed, active-user-authentication} & 62. Average distance between points & \cite{towards-continuous-passive, performance-analysis, explainability} & 84. Stdev end-to-end dev.   & \cite{performance-analysis}  \\
16. Direction of end-to-end line & \cite{touchalytics, towards-continuous-passive, information-revealed, power-consumption, posture-size-config, dakota} & 63. Stdev distance between points & \cite{towards-continuous-passive, performance-analysis} & 83. IQR end-to-end dev. & \cite{performance-analysis} \\
17. Average pairwise direction & \cite{touchalytics} & 64-68. LDP X,Y,area,pressure,velocity & \cite{towards-continuous-passive,behave-sense} & 85. Skewness of end-to-end dev. & \cite{performance-analysis} \\
\makecell[l]{18. Ratio of "end-to-end distance"\\ and "length of trajectory"} & \cite{touchalytics,  towards-continuous-passive, active-user-authentication, posture-size-config, dakota} & \makecell[l]{69-71. Start to LDP Latency,\\ Length, Direction} & \cite{towards-continuous-passive} & 86. Kurtosis of end-to-end dev.  & \cite{performance-analysis}  \\
19. 20\% perc. pairwise velocity & \cite{touchalytics, active-user-authentication, posture-size-config, dakota} & \makecell[l]{72-74. LDP to Stop Latency, Length,\\ Direction} & \cite{towards-continuous-passive} & 87. Average pairwise angle & \cite{performance-analysis} \\
20. 50\% perc.pairwise velocity & \cite{touchalytics, which-verifiers-work,  performance-analysis, active-user-authentication, posture-size-config, dakota} & & & 88. Median pairwise angle & \cite{performance-analysis} \\
21. 80\% perc. pairwise velocity & \cite{touchalytics, active-user-authentication, posture-size-config, dakota} & & & 89. Stdev pairwise angle & \cite{performance-analysis} \\
22. 20\% perc. pairwise accel & \cite{touchalytics, active-user-authentication, dakota} & & & 90. IQR pairwise angle & \cite{performance-analysis}  \\
23. 50\% perc. pairwise acceleration & \cite{touchalytics, which-verifiers-work,  performance-analysis, active-user-authentication, dakota} & & & 91. Skewness pairwise angle & \cite{performance-analysis} \\
24. 80\% perc. pairwise acceleration & \cite{touchalytics, active-user-authentication, dakota} & & & 92. Kurtosis pairwise angle & \cite{performance-analysis} \\
25. 20\% perc. end-to-end dev. & \cite{touchalytics, active-user-authentication} & & & 93. Average phase-angle & \cite{performance-analysis}  \\
26. 50\% perc. end-to-end dev. & \cite{touchalytics,  performance-analysis, active-user-authentication} & & & 94. Median phase-angle & \cite{performance-analysis}  \\
27. 80\% perc. end-to-end dev. & \cite{touchalytics, active-user-authentication} & & & 95. Stdev phase-angle & \cite{performance-analysis}  \\
28. Largest end-to-end dev. & \cite{touchalytics, information-revealed, active-user-authentication} & & & 96. IQR phase-angle & \cite{performance-analysis}  \\
29. Pressure at first point & \cite{unobservable-re-authentication, towards-continuous-passive} & & & 97. Skewness phase-angle & \cite{performance-analysis}  \\
30. Area at first point & \cite{unobservable-re-authentication, towards-continuous-passive} & & & 98. Kurtosis phase-angle & \cite{performance-analysis} \\
31. First moving direction & \cite{unobservable-re-authentication, towards-continuous-passive} & & & 99. Ratio of displacement to duration & \cite{performance-analysis} \\
32. Average moving direction & \cite{unobservable-re-authentication, information-revealed, active-user-authentication, dakota} & & & 100. IQR velocity & \cite{performance-analysis} \\
33. Average moving curvature & \cite{unobservable-re-authentication} & & & 101. Skewness velocity & \cite{performance-analysis} \\
34. Average curvature distance & \cite{unobservable-re-authentication} & & & 102. Kurtosis velocity & \cite{performance-analysis} \\
35. Average pressure & \cite{unobservable-re-authentication, which-verifiers-work, towards-continuous-passive,performance-analysis, power-consumption} & & & 103. Average anglular-velocity & \cite{performance-analysis} \\
36. Average touch area & \makecell[l]{\cite{unobservable-re-authentication, which-verifiers-work, towards-continuous-passive}\\ \cite{power-consumption, explainability, touch-pattern-isolation}} & & & 104. Median anglular-velocity & \cite{performance-analysis} \\
37. Max-area portion & \cite{unobservable-re-authentication} & & & 105. Stdev anglular-velocity & \cite{performance-analysis} \\
38. Min-pressure portion & \cite{unobservable-re-authentication} & & & 106. IQR anglular-velocity & \cite{performance-analysis} \\
& & & & 107. Skewness anglular-velocity & \cite{performance-analysis} \\
& & & & 108. Kurtosis anglular-velocity & \cite{performance-analysis} \\
& & & & 109. IQR acceleration & \cite{performance-analysis} \\
& & & & 110. Skewness acceleration & \cite{performance-analysis} \\
& & & & 111. Kurtosis acceleration & \cite{performance-analysis} \\
& & & & 112. IQR pressure & \cite{performance-analysis} \\
& & & & 113. Skewness pressure & \cite{performance-analysis} \\
& & & & 114. Kurtosis pressure & \cite{performance-analysis} \\
& & & & 115. Min pressure & \cite{towards-cont-passive, explainability} \\
& & & & 116. Max pressure & \cite{towards-cont-passive, explainability} \\
& & & & 117. Min area & \cite{towards-cont-passive, explainability} \\
& & & & 118. Max area & \cite{towards-cont-passive, explainability} \\
& & & & 119. Min velocity & \cite{towards-cont-passive, behave-sense} \\
& & & & 120. Max velocity & \cite{towards-cont-passive, behave-sense} \\
& & & & 121. Min pressure change & \cite{towards-cont-passive} \\
& & & & 122. Max pressure change & \cite{towards-cont-passive} \\
& & & & 123. Mean pressure change & \cite{towards-cont-passive} \\
& & & & 124. Median pressure change & \cite{towards-cont-passive} \\
& & & & 125. Min area change & \cite{towards-cont-passive} \\
& & & & 126. Max area change & \cite{towards-cont-passive} \\
& & & & 127. Mean area change & \cite{towards-cont-passive} \\
& & & & 128. Median area change & \cite{towards-cont-passive} \\
& & & & 129. X at max velocity & \cite{behave-sense} \\
& & & & 130. Y at max velocity & \cite{behave-sense} \\
& & & & 131. X at min velocity & \cite{behave-sense} \\
& & & & 132. Y at min velocity & \cite{behave-sense} \\
& & & & 133. Quadratic fit pressure x2 & \cite{explainability} \\
& & & & 134. Quadratic fit pressure x & \cite{explainability} \\
& & & & 135. Quadratic fit pressure n & \cite{explainability} \\
& & & & 136. Min time duration between points & \cite{explainability} \\
& & & & 137. Max time duration between points & \cite{explainability} \\
& & & & 138. Average time duration between points & \cite{explainability} \\
& & & & 139. Max deviation of mean X & \cite{dakota} \\
& & & & 140. Max deviation of mean Y & \cite{dakota} \\
& & & & 141. 20\% perc deviation of mean X & \cite{dakota} \\
& & & & 142. 20\% perc deviation of mean Y & \cite{dakota} \\
& & & & 143. Median deviation of mean X & \cite{dakota} \\
& & & & 144. Median deviation of mean Y & \cite{dakota} \\
& & & & 145. 80\% perc deviation of mean X & \cite{dakota} \\
& & & & 146. 80\% perc deviation of mean Y & \cite{dakota} \\
& & & & 147. Direction vector X & \cite{touch-pattern-isolation} \\
& & & & 148. Direction vector Y & \cite{touch-pattern-isolation} \\
& & & & 149. Horizontal/Vertical flag & \cite{posture-size-config} \\

\bottomrule
\end{tabular}
\end{table*}

